A quantum Fourier transform (QFT) based note detection algorithm

In quantum information processing (QIP), the quantum Fourier transform (QFT) has a plethora of applications [1] [2] [3]: Shor's algorithm and phase estimation are just a few well-known examples. Shor's quantum factorization algorithm, one of the most widely quoted quantum algorithms [4] [5] [6] relies heavily on the QFT and efficiently finds integer prime factors of large numbers on quantum computers [4]. This seminal ground-breaking design for quantum algorithms has triggered a cascade of viable alternatives to previously unsolvable problems on a classical computer that are potentially superior and can run in polynomial time. In this work we examine the QFT's structure and implementation for the creation of a quantum music note detection algorithm both on a simulated and a real quantum computer. Though formal approaches [7] [1] [8] [9] exist for the verification of quantum algorithms, in this study we limit ourselves to a simpler, symbolic representation which we validate using the symbolic SymPy [10] [11] package which symbolically replicates quantum computing processes. The algorithm is then implemented as a quantum circuit, using IBM's qiskit [12] library and finally period detection is exemplified on an actual single musical tone using a varying number of qubits.

==> custom_python_lang.tex <==
%\lstautogobble % to align correctly the left margin of code with text

\definecolor{halfgray}{gray}{0.55}
\definecolor{pyframe}{RGB}{207, 207, 207}
\definecolor{pybackground}{rgb}{0.95,0.95,0.95}
%\definecolor{ipython_red}{RGB}{186, 33, 33}
%\definecolor{pygreen}{RGB}{0, 128, 0}
%\definecolor{pygreen}{HTML}{064635}
%\definecolor{pycyan}{RGB}{64, 128, 128}
\definecolor{pypurple}{RGB}{170, 34, 255}

% strings
\definecolor{pykeyword}{HTML}{2A9D8F}
% keywords
\definecolor{pyblue}{HTML}{4062BB}
\definecolor{ipython_red}{HTML}{52489C}
% comments
\definecolor{pycyan}{HTML}{E76F51}

\lstdefinelanguage{Python}{
    morekeywords={access,and,as,assert,break,class,continue,def,del,elif,else,except,exec,finally,for,from,global,if,import,in,is,lambda,not,or,pass,print,raise,return,try,while},
    morekeywords=[2]{abs,all,any,basestring,bin,bool,bytearray,callable,chr,classmethod,cmp,compile,complex,delattr,dict,dir,divmod,enumerate,eval,execfile,file,filter,float,format,frozenset,getattr,globals,hasattr,hash,help,hex,id,input,int,isinstance,issubclass,iter,len,list,locals,long,map,max,memoryview,min,next,object,oct,open,ord,pow,property,range,raw_input,reduce,reload,repr,reversed,round,set,setattr,slice,sorted,staticmethod,str,sum,super,tuple,type,unichr,unicode,vars,xrange,zip,buffer,coerce,intern,True,False,self},
    sensitive=true,
    morecomment=[l]\#,
    morestring=[b]',
    morestring=[b]",
    morestring=[s]{'''}{'''},
    morestring=[s]{"""}{"""},
    morestring=[s]{r'}{'},
    morestring=[s]{r"}{"},
    morestring=[s]{r'''}{'''},
    morestring=[s]{r"""}{"""},
    morestring=[s]{u'}{'},
    morestring=[s]{u"}{"},
    morestring=[s]{u'''}{'''},
    morestring=[s]{u"""}{"""},
    % {replace}{replacement}{lenght of replace}
    % *{-}{-}{1} will not replace in comments and so on
    literate=
    {á}{{\'a}}1 {é}{{\'e}}1 {í}{{\'i}}1 {ó}{{\'o}}1 {ú}{{\'u}}1
    {Á}{{\'A}}1 {É}{{\'E}}1 {Í}{{\'I}}1 {Ó}{{\'O}}1 {Ú}{{\'U}}1
    {à}{{\`a}}1 {è}{{\`e}}1 {ì}{{\`i}}1 {ò}{{\`o}}1 {ù}{{\`u}}1
    {À}{{\`A}}1 {È}{{\'E}}1 {Ì}{{\`I}}1 {Ò}{{\`O}}1 {Ù}{{\`U}}1
    {ä}{{\"a}}1 {ë}{{\"e}}1 {ï}{{\"i}}1 {ö}{{\"o}}1 {ü}{{\"u}}1
    {Ä}{{\"A}}1 {Ë}{{\"E}}1 {Ï}{{\"I}}1 {Ö}{{\"O}}1 {Ü}{{\"U}}1
    {â}{{\^a}}1 {ê}{{\^e}}1 {î}{{\^i}}1 {ô}{{\^o}}1 {û}{{\^u}}1
    {Â}{{\^A}}1 {Ê}{{\^E}}1 {Î}{{\^I}}1 {Ô}{{\^O}}1 {Û}{{\^U}}1
    {œ}{{\oe}}1 {Œ}{{\OE}}1 {æ}{{\ae}}1 {Æ}{{\AE}}1 {ß}{{\ss}}1
    {ç}{{\c c}}1 {Ç}{{\c C}}1 {ø}{{\o}}1 {å}{{\r a}}1 {Å}{{\r A}}1
    {€}{{\EUR}}1 {£}{{\pounds}}1
    %
    {^}{{{\color{pypurple}\^{}}}}1
    {=}{{{\color{pypurple}=}}}1
    %
    {+}{{{\color{pypurple}+}}}1
    {*}{{{\color{pypurple}$^\ast$}}}1
    {/}{{{\color{pypurple}/}}}1
    %
    {+=}{{{+=}}}1
    {-=}{{{-=}}}1
    {*=}{{{$^\ast$=}}}1
    {/=}{{{/=}}}1,
    literate=
    *{-}{{{\color{pypurple}-}}}1
     {?}{{{\color{pypurple}?}}}1,
    %
    identifierstyle=\color{black}\ttfamily,
    commentstyle=\color{pycyan}\ttfamily,
    stringstyle=\color{ipython_red}\ttfamily,
    showstringspaces = false,
    keepspaces=true,
    showspaces=false,
    showstringspaces=false,
    rulecolor=\color{pyframe},
    frame=single,
    frameround={t}{t}{t}{t},
    framexleftmargin=6mm,
    numbers=left,
    numberstyle=\tiny\color{halfgray},
    backgroundcolor=\color{pybackground},
    % extendedchars=true,
    basicstyle=\ttfamily\smaller[0.5],
    keywordstyle=\color{pykeyword}\ttfamily,
    keywords=[3]{MCState,QGT, Ising, MetropolisLocal,MetropolisHamiltonian, MetropolisExchange,MetropolisRule, MetropolisSampler, ARDirectSampler, ExactSampler, GaussianRule,Sgd, Adam, Square, Spin, Chain, NDM, DeepSet, SR, Heisenberg, VMC, TDVP, Particle, KineticEnergy, PotentialEnergy,ContinuousOperator, MetropolisGaussian, Gaussian, RBMSymm, RBM, RBMModPhase, RBMMultiVal, GCNN, Triangular, Honeycomb, PointGroup, Graph, D, Lattice, Hypercube, sigmam, sigmap, LocalLiouvillian, MCMixedState, SteadyState, QGTJacobianPyTree, QGTJacobianDense, QGTOnTheFly,QGTJacobian, Heun, Euler, LocalOperator, Dense, Conv, Jastrow, ARNNSampler,ARNNDense, ARNNConv1D, ARNNConv2D, FastARNNConv1D, FastARNNConv2D,PermutationGroup,MetropolisExchange,MetropolisHamiltonian,ExactSampler,ARDirectSampler,ARNNDense,ARNNConv1D,ARNNConv2D,FastARNNConv1D,FastARNNConv2D,Jastrow,MultiLayerCNN,OneLayerNQS,FrozenDict,Pyrochlore,Identity,AbstractHilbert,Fock,ContinuousBoson,ContinuousHilbert,DiscreteHilbert,DeviceArray,Qubit,PRNGKey,DoubledHilbert,DiscreteOperator,PauliStrings,VariationalState,ExactState,SpaceGroupBuilder,Fd3m,LocalLiovillian,AbstractSampler,TwoLocalRule,Module},
    keywordstyle={[3]\color{pyblue}},
}

\lstset{
    language=Python,
    columns=fullflexible,
    breaklines=true,
    breakatwhitespace=true,
    extendedchars=true,
    breaklines=true, 
    xleftmargin=.05\textwidth, % experimentally determined . should fix
    columns=fullflexible,
    flexiblecolumns=true,
    literate=
    {á}{{\'a}}1 {é}{{\'e}}1 {í}{{\'i}}1 {ó}{{\'o}}1 {ú}{{\'u}}1
    {Á}{{\'A}}1 {É}{{\'E}}1 {Í}{{\'I}}1 {Ó}{{\'O}}1 {Ú}{{\'U}}1
    {à}{{\`a}}1 {è}{{\`e}}1 {ì}{{\`i}}1 {ò}{{\`o}}1 {ù}{{\`u}}1
    {À}{{\`A}}1 {È}{{\'E}}1 {Ì}{{\`I}}1 {Ò}{{\`O}}1 {Ù}{{\`U}}1
    {ä}{{\"a}}1 {ë}{{\"e}}1 {ï}{{\"i}}1 {ö}{{\"o}}1 {ü}{{\"u}}1
    {Ä}{{\"A}}1 {Ë}{{\"E}}1 {Ï}{{\"I}}1 {Ö}{{\"O}}1 {Ü}{{\"U}}1
    {â}{{\^a}}1 {ê}{{\^e}}1 {î}{{\^i}}1 {ô}{{\^o}}1 {û}{{\^u}}1
    {Â}{{\^A}}1 {Ê}{{\^E}}1 {Î}{{\^I}}1 {Ô}{{\^O}}1 {Û}{{\^U}}1
    {œ}{{\oe}}1 {Œ}{{\OE}}1 {æ}{{\ae}}1 {Æ}{{\AE}}1 {ß}{{\ss}}1
    {ç}{{\c c}}1 {Ç}{{\c C}}1 {ø}{{\o}}1 {å}{{\r a}}1 {Å}{{\r A}}1
    {€}{{\EUR}}1 {£}{{\pounds}}1 {σ}{{$\mathtt{\sigma}$}}1
    {\\\-}{}{0\discretionary{\textrm{-}}{}{}}
    %{.}{}{0\discretionary{.}{}{.}}% line-break at .
}

